Generalization of Quasi-Newton Methods: Application to Robust Symmetric Multisecant Updates

Quasi-Newton techniques approximate the Newton step by estimating the Hessian using the so-called secant equations. Some of these methods compute the Hessian using several secant equations but produce non-symmetric updates. Other quasi-Newton schemes, such as BFGS, enforce symmetry but cannot satisfy more than one secant equation. We propose a new type of quasi-Newton symmetric update using several secant equations in a least-squares sense. Our approach generalizes and unifies the design of quasi-Newton updates and satisfies provable robustness guarantees.

==> utils/utils_optml.tex <==

\usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{amssymb}
\usepackage{empheq}
\usepackage{xcolor, color, colortbl}
\usepackage{framed}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{enumitem}
% For figures
\usepackage{graphicx} % more modern
%\usepackage{epsfig} % less modern

% to avoid too much space after the algorithm
% \setlength{\textfloatsep}{10pt}% Remove \textfloatsep

\usepackage{nicefrac}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{nccmath}

\usepackage[tikz]{bclogo}
\usepackage{wasysym}

%\SetAlFnt{\normalsize}

\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
% \usepackage[
%     linkcolor=mydarkblue,
%     citecolor=mydarkblue,
%     filecolor=mydarkblue,
%     urlcolor=mydarkblue,
%     pdfview=FitH]{hyperref}

% smaller url fonts
\usepackage{url}
\usepackage{relsize}
\renewcommand*{\UrlFont}{\ttfamily\smaller\relax}

\newcommand{\blue}{\color{blue}}
\def\xx{\textbf{x}}
\def\yy{\textbf{y}}
\def\zz{\textbf{z}}
\def\qq{\textbf{q}}
\def\dd{\textbf{d}}
\def\XX{\textbf{X}}
\def\YY{\textbf{Y}}
\def\ZZ{\textbf{Z}}
\def\aa{\textbf{a}}
\def\bb{\textbf{b}}
\def\rr{\textbf{r}}
\def\cc{\textbf{c}}
\def\qq{\textbf{q}}
\def\WW{\textbf{W}}
\def\KK{\textbf{K}}
\def\II{\textbf{I}}
\def\yy{\textbf{y}}
\def\vv{\textbf{v}}
\def\uu{\textbf{u}}
\def\ww{\textbf{w}}
\def\zz{\textbf{z}}
\def\SS{\textbf{S}}
\def\BB{\textbf{B}}
\def\AA{\textbf{A}}
\def\CC{\textbf{C}}
\def\MM{\textbf{M}}
\def\CC{\textbf{C}}
\def\DD{\textbf{D}}
\def\GG{\textbf{G}}
\def\PP{\textbf{P}}
\def\TT{\textbf{T}}
\def\VV{\textbf{V}}
\def\QQ{\textbf{Q}}
\def\UU{\textbf{U}}
\def\HH{\textbf{H}}
\def\EE{\textbf{E}}
\def\bSigma{{\boldsymbol \Sigma}}
\def\zzref{\textbf{z}_{\text{ref}}}

\def\dA{\delta_{\boldsymbol A}}
\def\dD{\delta_{\boldsymbol D}}

\def\bphi{{\boldsymbol \phi}}
\def\balpha{{\boldsymbol \alpha}}
\def\bpsi{{\boldsymbol \psi}}
\def\LLambda{{\boldsymbol \Lambda}}
\def\eeps{{\boldsymbol \varepsilon}}
\def\dif{\mathop{}\!\mathrm{d}}
\def\Proba{\mathbb{P}}
\def\MP{\mu_{\mathrm{MP}}}


\def\calR{\mathcal{R}}
\def\calC{\mathcal{C}}
\def\calL{\mathcal{L}}


\def\HHref{{\HH}_{\text{ref}}}
\def\BBref{{\BB}_{\text{ref}}}
\def\MMref{{\MM}_{\text{ref}}}
\def\ZZref{{\ZZ}_{\text{ref}}}


\def\RR{{\mathbb R}}
\def\R{{\mathbb R}}
\newcommand{\Econd}{\mathbf{E}}
\renewcommand{\gg}{\boldsymbol{g}}
\renewcommand{\vec}{\mathbf{vec}}
\DeclareMathOperator{\prox}{\mathbf{prox}}
\DeclareMathOperator{\tr}{tr}
\def\defas{\stackrel{\text{def}}{=}}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator*{\Fix}{Fix}
\DeclareMathOperator*{\Var}{Var}
\DeclareMathOperator*{\Span}{\mathbf{span}}
\DeclareMathOperator*{\Deg}{{deg}}
\DeclareMathOperator*{\Trace}{{tr}}
\DeclareMathOperator*{\rank}{\mathbf{rank}}

\newcommand{\Pone}[1]{\mathcal{P}_{#1}^{(1)}}

% \newcommand{\xdownarrow}[1]{%
%   {\left\downarrow\vbox to #1{}\right.\kern-\nulldelimiterspace}
% }


\newcommand*\mybluebox[1]{\colorbox{myblue}{\hspace{1em}#1\hspace{1em}}}

\DeclareMathOperator*{\argmin}{{arg\,min}}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\diag}{\mathbf{diag}}

\newcommand{\norm}[1]{\|#1\|}

\definecolor{myblue}{HTML}{D2E4FC}
\definecolor{Gray}{gray}{0.92}
    
\newtheorem{assumption}{Assumption}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary }


\usepackage{thmtools}
\usepackage{thm-restate}

\usepackage{wrapfig}

\declaretheorem[name=Theorem,numberwithin=section]{thm}
\declaretheorem[name=Proposition,numberwithin=section]{prop}


\newcommand{\DX}{\Delta\XX}
\newcommand{\DG}{\Delta\GG}


\usepackage{algorithmic,algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


